DCPViz: A Visual Analytics Approach for Downscaled Climate Projections

This paper introduces a novel visual analytics approach, DCPViz, to enable climate scientists to explore massive climate data interactively without requiring the upfront movement of massive data. Thus, climate scientists are afforded more effective approaches to support the identification of potential trends and patterns in climate projections and their subsequent impacts. We designed the DCPViz pipeline to fetch and extract NEX-DCP30 data with minimal data transfer from their public sources. We implemented DCPViz to demonstrate its scalability and scientific value and to evaluate its utility under three use cases based on different models and through domain expert feedback.

==> sections/default.tex <==
\section{Using the Style Template}

% \begin{itemize}
% \item If you receive compilation errors along the lines of ``\texttt{Package ifpdf Error: Name clash, \textbackslash ifpdf is already defined}'' then please add a new line ``\texttt{\textbackslash let\textbackslash ifpdf\textbackslash relax}'' right after the ``\texttt{\textbackslash documentclass[journal]\{vgtc\}}'' call. Note that your error is due to packages you use that define ``\texttt{\textbackslash ifpdf}'' which is obsolete (the result is that \texttt{\textbackslash ifpdf} is defined twice); these packages should be changed to use ifpdf package instead.
% \item Note that each author's affiliations have to be provided in the author footer on the bottom-left corner of the first page. It is permitted to merge two or more people from the same institution as long as they are shown in the same order as in the overall author sequence on the top of the first page. For example, if authors A, B, C, and D are from institutions 1, 2, 1, and 2, respectively, then it is ok to use 2 bullets as follows:
% \begin{itemize}
% \item A and C are with Institution 1. E-mail: \{a\,$|$\,c\}@i1.com\,.
% \item B and D are with Institution 2. E-mail: \{b\,$|$\,d\}@i2.org\,.
% \end{itemize}
% \item The style uses the hyperref package, thus turns references into internal links. We thus recommend to make use of the ``\texttt{\textbackslash autoref\{reference\}}'' call (instead of ``\texttt{Figure\~{}\textbackslash ref\{reference\}}'' or similar) since ``\texttt{\textbackslash autoref\{reference\}}'' turns the entire reference into an internal link, not just the number. Examples: \autoref{fig:sample} and \autoref{tab:vis_papers}.
% \item The style automatically looks for image files with the correct extension (eps for regular \LaTeX; pdf, png, and jpg for pdf\LaTeX), in a set of given subfolders (figures/, pictures/, images/). It is thus sufficient to use ``\texttt{\textbackslash includegraphics\{CypressView\}}'' (instead of ``\texttt{\textbackslash includegraphics\{pictures/CypressView.jpg\}}'').
% \item For adding hyperlinks and DOIs to the list of references, you can use ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-hyperref-narrow\}}'' (instead of ``\texttt{\textbackslash bibliographystyle\{abbrv\}}''). It uses the doi and url fields in a bib\TeX\ entry and turns the entire reference into a link, giving priority to the doi. The doi can be entered with or without the ``\texttt{http://dx.doi.org/}'' url part. See the examples in the bib\TeX\ file and the bibliography at the end of this template.\\[1em]
% \textbf{Note 1:} occasionally (for some \LaTeX\ distributions) this hyper-linked bib\TeX\ style may lead to \textbf{compilation errors} (``\texttt{pdfendlink ended up in different nesting level ...}'') if a reference entry is broken across two pages (due to a bug in hyperref). In this case make sure you have the latest version of the hyperref package (i.\,e., update your \LaTeX\ installation/packages) or, alternatively, revert back to ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-narrow\}}'' (at the expense of removing hyperlinks from the bibliography) and try ``\texttt{\textbackslash bibliographystyle\{abbrv-doi-hyperref-narrow\}}'' again after some more editing.\\[1em]
% \textbf{Note 2:} the ``\texttt{-narrow}'' versions of the bibliography style use the font ``PTSansNarrow-TLF'' for typesetting the DOIs in a compact way. This font needs to be available on your \LaTeX\ system. It is part of the \href{https://www.ctan.org/pkg/paratype}{``paratype'' package}, and many distributions (such as MikTeX) have it automatically installed. If you do not have this package yet and want to use a ``\texttt{-narrow}'' bibliography style then use your \LaTeX\ system's package installer to add it. If this is not possible you can also revert to the respective bibliography styles without the ``\texttt{-narrow}'' in the file name.\\[1em]
% DVI-based processes to compile the template apparently cannot handle the different font so, by default, the template file uses the \texttt{abbrv-doi} bibliography style but the compiled PDF shows you the effect of the \texttt{abbrv-doi-hyperref-narrow} style.
% \end{itemize}

% \section{Bibliography Instructions}

% \begin{itemize}
% \item Sort all bibliographic entries alphabetically but the last name of the first author. This \LaTeX/bib\TeX\ template takes care of this sorting automatically.
% \item Merge multiple references into one; e.\,g., use \cite{Max:1995:OMF,Kitware:2003} (not \cite{Kitware:2003}\cite{Max:1995:OMF}). Within each set of multiple references, the references should be sorted in ascending order. This \LaTeX/bib\TeX\ template takes care of both the merging and the sorting automatically.
% \item Verify all data obtained from digital libraries, even ACM's DL and IEEE Xplore  etc.\ are sometimes wrong or incomplete.
% \item Do not trust bibliographic data from other services such as Mendeley.com, Google Scholar, or similar; these are even more likely to be incorrect or incomplete.
% \item Articles in journal---items to include:
%   \begin{itemize}
%   \item author names
% 	\item title
% 	\item journal name
% 	\item year
% 	\item volume
% 	\item number
% 	\item month of publication as variable name (i.\,e., \{jan\} for January, etc.; month ranges using \{jan \#\{/\}\# feb\} or \{jan \#\{-{}-\}\# feb\})
%   \end{itemize}
% \item use journal names in proper style: correct: ``IEEE Transactions on Visualization and Computer Graphics'', incorrect: ``Visualization and Computer Graphics, IEEE Transactions on''
% \item Papers in proceedings---items to include:
%   \begin{itemize}
%   \item author names
% 	\item title
% 	\item abbreviated proceedings name: e.\,g., ``Proc.\textbackslash{} CONF\_ACRONYNM'' without the year; example: ``Proc.\textbackslash{} CHI'', ``Proc.\textbackslash{} 3DUI'', ``Proc.\textbackslash{} Eurographics'', ``Proc.\textbackslash{} EuroVis''
% 	\item year
% 	\item publisher
% 	\item town with country of publisher (the town can be abbreviated for well-known towns such as New York or Berlin)
%   \end{itemize}
% \item article/paper title convention: refrain from using curly brackets, except for acronyms/proper names/words following dashes/question marks etc.; example:
% \begin{itemize}
% 	\item paper ``Marching Cubes: A High Resolution 3D Surface Construction Algorithm''
% 	\item should be entered as ``\{M\}arching \{C\}ubes: A High Resolution \{3D\} Surface Construction Algorithm'' or  ``\{M\}arching \{C\}ubes: A high resolution \{3D\} surface construction algorithm''
% 	\item will be typeset as ``Marching Cubes: A high resolution 3D surface construction algorithm''
% \end{itemize}
% \item for all entries
% \begin{itemize}
% 	\item DOI can be entered in the DOI field as plain DOI number or as DOI url; alternative: a url in the URL field
% 	\item provide full page ranges AA-{}-BB
% \end{itemize}
% \item when citing references, do not use the reference as a sentence object; e.\,g., wrong: ``In \cite{Lorensen:1987:MCA} the authors describe \dots'', correct: ``Lorensen and Cline \cite{Lorensen:1987:MCA} describe \dots''
% \end{itemize}

% \section{Example Section}

% Lorem\marginpar{\small You can use the margins for comments while editing the submission, but please remove the marginpar comments for submission.} ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
% nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
% sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
% rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
% ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
% sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
% dolore magna aliquyam erat, sed diam
% voluptua~\cite{Kitware:2003,Max:1995:OMF}. At vero eos et accusam et
% justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
% takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
% amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
% invidunt ut labore et dolore magna aliquyam erat, sed diam
% voluptua. At vero eos et accusam et justo duo dolores et ea
% rebum. Stet clita kasd gubergren, no sea takimata sanctus est.

% \section{Exposition}

% Duis autem vel eum iriure dolor in hendrerit in vulputate velit esse
% molestie consequat, vel illum dolore eu feugiat nulla facilisis at
% vero eros et accumsan et iusto odio dignissim qui blandit praesent
% luptatum zzril delenit augue duis dolore te feugait nulla
% facilisi. Lorem ipsum dolor sit amet, consectetuer adipiscing elit,
% sed diam nonummy nibh euismod tincidunt ut laoreet dolore magna
% aliquam erat volutpat~\cite{Kindlmann:1999:SAG}.

% \begin{equation}
% \sum_{j=1}^{z} j = \frac{z(z+1)}{2}
% \end{equation}

% Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
% nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
% sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
% rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
% ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
% sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
% dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
% et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
% takimata sanctus est Lorem ipsum dolor sit amet.

% \subsection{Lorem ipsum}

% Lorem ipsum dolor sit amet (see \autoref{tab:vis_papers}), consetetur sadipscing elitr, sed diam
% nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
% sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
% rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
% ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
% sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
% dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
% et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
% takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
% amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
% invidunt ut labore et dolore magna aliquyam erat, sed diam
% voluptua. At vero eos et accusam et justo duo dolores et ea
% rebum. 

% \begin{table}[tb]
%   \caption{VIS/VisWeek accepted/presented papers: 1990--2016.}
%   \label{tab:vis_papers}
%   \scriptsize%
% 	\centering%
%   \begin{tabu}{%
% 	r%
% 	*{7}{c}%
% 	*{2}{r}%
% 	}
%   \toprule
%   year & \rotatebox{90}{Vis/SciVis} &   \rotatebox{90}{SciVis conf} &   \rotatebox{90}{InfoVis} &   \rotatebox{90}{VAST} &   \rotatebox{90}{VAST conf} &   \rotatebox{90}{TVCG @ VIS} &   \rotatebox{90}{CG\&A @ VIS} &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{incl. TVCG/CG\&A}   &   \rotatebox{90}{VIS/VisWeek} \rotatebox{90}{w/o TVCG/CG\&A}   \\
%   \midrule
% 	2016 & 30 &   & 37 & 33 & 15 & 23 & 10 & 148 & 115 \\
%   2015 & 33 & 9 & 38 & 33 & 14 & 17 & 15 & 159 & 127 \\
%   2014 & 34 &   & 45 & 33 & 21 & 20 &   & 153 & 133 \\
%   2013 & 31 &   & 38 & 32 &   & 20 &   & 121 & 101 \\
%   2012 & 42 &   & 44 & 30 &   & 23 &   & 139 & 116 \\
%   2011 & 49 &   & 44 & 26 &   & 20 &   & 139 & 119 \\
%   2010 & 48 &   & 35 & 26 &   &   &   & 109 & 109 \\
%   2009 & 54 &   & 37 & 26 &   &   &   & 117 & 117 \\
%   2008 & 50 &   & 28 & 21 &   &   &   & 99 & 99 \\
%   2007 & 56 &   & 27 & 24 &   &   &   & 107 & 107 \\
%   2006 & 63 &   & 24 & 26 &   &   &   & 113 & 113 \\
%   2005 & 88 &   & 31 &   &   &   &   & 119 & 119 \\
%   2004 & 70 &   & 27 &   &   &   &   & 97 & 97 \\
%   2003 & 74 &   & 29 &   &   &   &   & 103 & 103 \\
%   2002 & 78 &   & 23 &   &   &   &   & 101 & 101 \\
%   2001 & 74 &   & 22 &   &   &   &   & 96 & 96 \\
%   2000 & 73 &   & 20 &   &   &   &   & 93 & 93 \\
%   1999 & 69 &   & 19 &   &   &   &   & 88 & 88 \\
%   1998 & 72 &   & 18 &   &   &   &   & 90 & 90 \\
%   1997 & 72 &   & 16 &   &   &   &   & 88 & 88 \\
%   1996 & 65 &   & 12 &   &   &   &   & 77 & 77 \\
%   1995 & 56 &   & 18 &   &   &   &   & 74 & 74 \\
%   1994 & 53 &   &   &   &   &   &   & 53 & 53 \\
%   1993 & 55 &   &   &   &   &   &   & 55 & 55 \\
%   1992 & 53 &   &   &   &   &   &   & 53 & 53 \\
%   1991 & 50 &   &   &   &   &   &   & 50 & 50 \\
%   1990 & 53 &   &   &   &   &   &   & 53 & 53 \\
%   \midrule
%   \textbf{sum} & \textbf{1545} & \textbf{9} & \textbf{632} & \textbf{310} & \textbf{50} & \textbf{123} & \textbf{25} & \textbf{2694} & \textbf{2546} \\
%   \bottomrule
%   \end{tabu}%
% \end{table}

% \subsection{Mezcal Head}

% Lorem ipsum dolor sit amet (see \autoref{fig:sample}), consetetur sadipscing elitr, sed diam
% nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
% sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
% rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
% ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
% sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
% dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
% et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
% takimata sanctus est Lorem ipsum dolor sit amet. 

% \subsubsection{Duis Autem}

% Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
% nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
% sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
% rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
% ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
% sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
% dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
% et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
% takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
% amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
% invidunt ut labore et dolore magna aliquyam erat, sed diam
% voluptua. At vero eos et accusam et justo duo dolores et ea
% rebum. Stet clita kasd gubergren, no sea takimata sanctus est. Lorem
% ipsum dolor sit amet.

% \begin{figure}[tb]
%  \centering % avoid the use of \begin{center}...\end{center} and use \centering instead (more compact)
%  \includegraphics[width=\columnwidth]{paper-count-w-2015-new}
%  \caption{A visualization of the 1990--2015 data from \autoref{tab:vis_papers}. The image is from \cite{Isenberg:2017:VMC} and is in the public domain.}
%  \label{fig:sample}
% \end{figure}

% \subsubsection{Ejector Seat Reservation}

% Duis autem~\cite{Lorensen:1987:MCA}\footnote{The algorithm behind
% Marching Cubes \cite{Lorensen:1987:MCA} had already been
% described by Wyvill et al. \cite{Wyvill:1986:DSS} a year
% earlier.} vel eum iriure dolor in hendrerit
% in vulputate velit esse molestie consequat,\footnote{Footnotes
% appear at the bottom of the column.} vel illum dolore eu
% feugiat nulla facilisis at vero eros et accumsan et iusto odio
% dignissim qui blandit praesent luptatum zzril delenit augue duis
% dolore te feugait nulla facilisi. Lorem ipsum dolor sit amet,
% consectetuer adipiscing elit, sed diam nonummy nibh euismod tincidunt
% ut laoreet dolore magna aliquam erat volutpat.


% \paragraph{Confirmed Ejector Seat Reservation}

% Ut wisi enim ad minim veniam, quis nostrud exerci tation ullamcorper
% suscipit lobortis nisl ut aliquip ex ea commodo
% consequat~\cite{Nielson:1991:TAD}. Duis autem vel eum iriure dolor in
% hendrerit in vulputate velit esse molestie consequat, vel illum dolore
% eu feugiat nulla facilisis at vero eros et accumsan et iusto odio
% dignissim qui blandit praesent luptatum zzril delenit augue duis
% dolore te feugait nulla facilisi.

% \paragraph{Rejected Ejector Seat Reservation}

% Ut wisi enim ad minim veniam, quis nostrud exerci tation ullamcorper
% suscipit lobortis nisl ut aliquip ex ea commodo consequat. Duis autem
% vel eum iriure dolor in hendrerit in vulputate velit esse molestie

% \subsection{Vestibulum}

% Vestibulum ut est libero. Suspendisse non libero id massa congue egestas nec at ligula. Donec nibh lorem, ornare et odio eu, cursus accumsan felis. Pellentesque habitant morbi tristique senectus et netus et malesuada fames ac turpis egestas. Donec dapibus quam vel eros mattis, id ornare dolor convallis. Donec at nisl sapien. Integer fringilla laoreet tempor. Fusce accumsan ante vel augue euismod, sit amet maximus turpis mattis. Nam accumsan vestibulum rhoncus. Aenean quis pellentesque augue. Suspendisse sed augue et velit consequat bibendum id nec est. Quisque erat purus, ullamcorper ut ex vel, dapibus dignissim erat.

% Quisque sit amet orci quam. Lorem ipsum dolor sit amet, consectetur adipiscing elit. Aliquam pharetra, nunc non efficitur convallis, tellus purus iaculis lorem, nec ultricies dolor ligula in metus. Class aptent taciti sociosqu ad litora torquent per conubia nostra, per inceptos himenaeos. Aenean eu ex nulla. Morbi id ex interdum, scelerisque lorem nec, iaculis dui. Phasellus ultricies nunc vitae quam fringilla laoreet. Quisque sed dolor at sem vestibulum fringilla nec ac augue. Ut consequat, velit ac mattis ornare, eros arcu pellentesque erat, non ultricies libero metus nec mi. Sed eget elit sed quam malesuada viverra. Quisque ullamcorper, felis ut convallis fermentum, purus ligula varius ligula, sit amet tempor neque dui non neque. Donec vulputate ultricies tortor in mollis.

% Integer sit amet dolor sit amet turpis ullamcorper varius. Cras volutpat bibendum scelerisque. Maecenas mauris dolor, gravida eu elit et, sodales consequat tortor. Integer id commodo elit. Pellentesque sollicitudin ex non nulla molestie eleifend. Mauris sagittis metus nec turpis imperdiet, vel ullamcorper nibh tincidunt. Sed semper tempus ex, ut aliquet erat hendrerit id. Maecenas sit amet dolor sollicitudin, luctus nunc sit amet, malesuada justo.

% Mauris ut sapien non ipsum imperdiet sodales sit amet ac diam. Nulla vel convallis est. Etiam dapibus augue urna. Aenean enim leo, fermentum quis pulvinar at, ultrices quis enim. Sed placerat porta libero et feugiat. Phasellus ullamcorper, felis id porta sollicitudin, dolor dui venenatis augue, vel fringilla risus massa non risus. Maecenas ut nulla vitae ligula pharetra feugiat non eu ante. Donec quis neque quis lorem cursus pretium ac vulputate quam. Cras viverra tellus vitae sapien pretium laoreet. Pellentesque fringilla odio venenatis ex viverra, quis eleifend tortor ornare. Ut ut enim nunc. Vivamus id ligula nec est dignissim eleifend.

% Nunc ac velit tellus. Donec et venenatis mauris. Lorem ipsum dolor sit amet, consectetur adipiscing elit. Ut vitae lectus vel ante mollis congue. Vestibulum at cursus velit. Curabitur in facilisis enim. Vestibulum eget dui aliquet risus laoreet laoreet. Phasellus et est id magna interdum venenatis. Donec luctus vehicula justo sed laoreet. Quisque tincidunt suscipit augue, in molestie sem accumsan sed.
% \section{Conclusion}

% Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam
% nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat,
% sed diam voluptua. At vero eos et accusam et justo duo dolores et ea
% rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem
% ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur
% sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et
% dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam
% et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea
% takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit
% amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor
% invidunt ut labore et dolore magna aliquyam erat, sed diam
% voluptua. At vero eos et accusam et justo duo dolores et ea
% rebum.


==> vis-metadata/README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> vis-metadata/makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

